Approaches of near stars to the Sun

We investigate aspects of computing the perihelion distances and impact parameters for near stars to the Sun, and, we analyze the solar motion. Keywords: perihelion distance, impact parameter, Oort cloud, solar motion

==> Chapter2.tex <==

\chapter{The Problem}
%\chaptermark{The problem}
We study the evolution of the Oort cloud of comets situated at the borders of the Solar System.
The comet motion with respect to the Sun is calculated on the basis of gravitational forces
acting both on the Sun and the comet. Effect of the Galaxy in the form of galactic tide
is based on the observations. The flat rotation curve is considered together with the
most probable values of the Oort constants. The effect of the galactic bulge is consistent
with the mass distribution given by Maoz(2007) \cite{maoz}. Moreover, motion of the Sun in the Galaxy
is considered, too. We take into account not only the fact that the Sun revolves the center of the Galaxy,
as it is conventionally done. We take into account also the oscillations of the Sun with respect
to the galactic equatorial plane. This model is presented in Kla\v{c}ka(2009) \cite{galaxy}. 
Besides the fixed mass density used as an approximation to reality for the galactic bulge,
we can take into account the decrease of the bulge mass density as a function of the distance
from the galactic equatorial plane. The effect of this simple improvement will be treated.
Great part of the Thesis will be devoted to the effect of close approaches of stars
or interstellar clouds to the Solar System. 

As for the last problem, we will first calculate impact parameter for a star with close
approach to the Solar system. Better value of the perihelion will be found using
the two body problem (the star and the Sun). \\
... two body problem + Galaxy
... two body problem + Galaxy + motion of the Sun with respect to galactic equatorial plane
... previous + motion of a comet with respect to the Sun .... various initial conditions for the comet \\

How can these effects enhance the number of comets entering the inner part of the Solar System?


==> chapter8.tex <==
\chapter{Conclusions}
\label{chapter.6}
\subsection{The perihelion distances}

\subsection{The solar motion}
We have calculated the solar motion with respect to three different
sets of stars using direct calculation and the approximative Least
square method. We can see in subsections \ref{s.1}, \ref{s.2} and
\ref{s.3} that, the solar motion depends on the number of stars in
our sample and their heliocentric distances. Our results correspond
to the standard solar motion.

Our Least square method offered six independent systems of linear
equations for the components $X_{S}$, $Y_{S}$ and $Z_{S}$ of the
solar motion. The systems containing two of the three velocity
components of the stars yield results for $X_{S}$, $Y_{S}$ and
$Z_{S}$ not consistent with the values found by the direct method.
However, also the systems of linear equations containing only one of the
observed velocity components (radial velocity of the $i-$th star,
its proper motions $\mu_{\alpha, i}$ and $\mu_{\delta, i}$) yield result
which may differ in more than 80\% from the direct method.
This is probably caused by the approximation given by Eq.~(\ref{eq.16}). 
However, the same approximation yields acceptable results for the cases when
only one of the velocity components of the stars (either radial
velocity, or proper motion in right ascension, or proper motion in
declination) is used. In any case, we can conclude that the Least square method 
is not a physical method for finding the solar motion. 

The value of $Z_{S}$ which we have found from the direct calculation
fulfills the condition $Z_{S}$ $\in$ $\langle 6.14, 7.70 \rangle$
$km~s^{-1}$. The values are consistent with the values presented by
other authors. However, our value of $V_{S}$ is larger than the
presented by other authors.

The nonzero values of $Z_{S}$ are important in determining the
largest distances of the Sun from the galactic equatorial plane. The
results are summarized in Tables ~\ref{t.5} and ~\ref{t.1}. Moreover, the values of
$Z_{S}$ are relevant in long-term evolution of comets of the Oort
cloud. Using the newest form of the galactic tides, the orbital
evolution of cometary orbital elements strongly depends on the value
of $Z_{S}$. The cometary orbital evolution significantly differs
from the results obtained by standard approach assuming a fixed
Sun's position in the galactic equatorial plane.

%In order to verify different methods of finding the solar motion, our sets contain only stars with complete observational data.
%Thus, we were able to compare the approximative methods using Least square method with the direct computation without any neglections.

We have chosen only stars with the best quality index (A) in
parallax, proper motions and radial velocities \cite{simbad}, that
minimized the influences of measurement errors. As we can see in
Table ~\ref{t.1}, our results from direct calculation are in
agreement with the standard solar motion presented in Table ~\ref{t.7}. Next, 
results in Table ~\ref{t.7} obviously ensure that the solar motion depends
on the stellar type. However, we want to know the solar
motion regardless of the stellar type. Hence we did not separate
stellar types in our calculations.

The direct method for finding solar motion yields that the direction
of the solar motion is characterized by the ecliptic longitude 
$\lambda$ $=$ 277.5$^{\circ}$ and latitude $\beta$ $=$ 60.3$^{\circ}$
(based on the values of Table ~\ref{t.4} for stars with distances less than 100 $pc$).
The solar motion was determined by the motion of the Sun with respect 
to the surrounding stars. The obtained direction may be compared
with the direction of the interstellar gas and dust streaming into the Solar System:
$\lambda$ $=$ 259$^{\circ}$ and $\beta$ $=$ 8$^{\circ}$.
The solar motion based on the surrounding stars yields $Z_{S}$
$\in$ $\langle$ 6.14 $km/s$, 7.70 $km/s$ $\rangle$. The solar motion
based on the surrounding dust and gas yields, approximately, 
$Z_{S}$ $\in$ $\langle$ 6.1 $km/s$, 6.5 $km/s$ $\rangle$.
In application to orbital evolution of a comet from the Oort cloud
we come to the conclusion that the number of cometary returns
into the inner part of the Solar System is twice the conventional value.

The knowledge of the solar motion allows to simulate the solar
motion with respect to galactic center. Especially $Z_S$, which
represents the solar motion in direction perpendicular to the
galactic equator, is used as a starting condition in simulation of
solar oscillations.

The uncertainty in the value of $Z_{S}$, $Z_{S}$ $\in$ $\langle$ 6.14 $km/s$, 7.70 $km/s$ $\rangle$,
would lead to the uncertainty in the mass of the Oort cloud of comets.
The uncertainty of the latter is greater than the uncertainty in $Z_{S}$.
A decrease in $Z_{S}$ in 20\% leads to the decrease of mass of the Oort cloud
in more than 30\%.
However, if also the results for interstellar gas and dust are taken into account, then
the lower value of $Z_{S}$ should be preferred.
This case yields that the frequency of cometary returns into the inner part 
of the Solar System is 1.33-times greater than the number for $Z_{S} \geq$
7.3 $km.s^{-1}$ (approximately), and 2-times greater than the frequency of the 
conventional models of the galactic tides. 

